Transformer-Enhanced Iterative Feedback Mechanism for Polyp Segmentation

Colorectal cancer (CRC) is the third most common cause of cancer diagnosed in the United States and the second leading cause of cancer-related death among both genders. Notably, CRC is the leading cause of cancer in younger men less than 50 years old. Colonoscopy is considered the gold standard for the early diagnosis of CRC. Skills vary significantly among endoscopists, and a high miss rate is reported. Automated polyp segmentation can reduce the missed rates, and timely treatment is possible in the early stage. To address this challenge, we introduce \textit{\textbf{\ac{FANetv2}}}, an advanced encoder-decoder network designed to accurately segment polyps from colonoscopy images. Leveraging an initial input mask generated by Otsu thresholding, FANetv2 iteratively refines its binary segmentation masks through a novel feedback attention mechanism informed by the mask predictions of previous epochs. Additionally, it employs a text-guided approach that integrates essential information about the number (one or many) and size (small, medium, large) of polyps to further enhance its feature representation capabilities. This dual-task approach facilitates accurate polyp segmentation and aids in the auxiliary classification of polyp attributes, significantly boosting the model's performance. Our comprehensive evaluations on the publicly available BKAI-IGH and CVC-ClinicDB datasets demonstrate the superior performance of FANetv2, evidenced by high dice similarity coefficients (DSC) of 0.9186 and 0.9481, along with low Hausdorff distances of 2.83 and 3.19, respectively. The source code for FANetv2 is available at https://github.com/xxxxx/FANetv2.

==> takeout.tex <==
% @article{silva2014toward,
%   title={Toward embedded detection of polyps in wce images for early diagnosis of colorectal cancer},
%   author={Silva, Juan and Histace, Aymeric and Romain, Olivier and Dray, Xavier and Granado, Bertrand},
%   journal={International journal of computer assisted radiology and surgery},
%   volume={9},
%   number={2},
%   pages={283--293},
%   year={2014}
% }


% Colonoscopy is a gold standard procedure but is highly operator-dependent. Automated semantic segmentation of polyps, a precancerous precursor, can minimize missed rates and timely treatment of colorectal-related cancer at early stage. Even though there are deep learning methods steered for this task, variability in polyp size can impact model training thereby limiting it to the attribute of the majority of samples present in the training dataset that may provide sub-optimal results to a differently sized polyp. What if we exploit the size-related features in the form of text attention during training? This process can enable disentanglement of differently sized polyps already at the first few-layers of the network that will further enable feature weights at subsequent layers to adjust. Our experimental results demonstrate that such added text embedding improves overall performance of the model compared to state-of-the-art segmentation methods. In addition, our proposed  can generalize well to variable sized polyps in different datasets. We explore five different datasets and provide insights for size-specific improvements.
% Clinical motivation
% Literature basics
% Novelty of the work
% Experiments

% Ablations?
% Removing text 
% Removing layers? B2 block?
% Public datasets {Kvasir-SEG, BKAI-IGH NeoPolyp, Kvasir-Sessile, ETIS-Larib}


%All models are trained on NVIDIA GeForce RTX 3090 GPU. Before being trained, we resized all four datasets to $256 \times 256$ pixels and split them into training, validation and testing sets with a ratio of 80:10:10, except Kvasir-SEG, for which we have adopted the official split of 880/120 for training and testing respectively. We use a simple and efficient data augmentation strategy by using augmentations such as random rotation, vertical flipping, horizontal flipping, and coarse dropout. We have trained all the models on a similar configuration of hyperparameters for each dataset conisisting of Adam optimizer with a learning rate of 1e-4. We have used a batch size of 16 and an early stopping mechanism and ReduceLROnPlateau to prevent the models from overfitting.  


%Additionally, we present algorithm complexity, such as the number of trainable parameters and flops used by the methods.  

%From Table~\ref{tab:results} and Table~\ref{tganet-effect}, it can be observed that {TGANet} model consistently segment polyps with the more precise area and boundary, which shows the robustness and superiority of the proposed model. Although DeepLabV3+~\cite{chen2018encoder} and PraNet~\cite{fan2020pranet} showed the competitive results with some datasets, however, their performance were not consistent. Additionally, our method is more efficient in terms of the number of trainable parameters and flops (GMac) as compared to both DeepLabv3+~\cite{chen2018encoder} and PraNet~\cite{fan2020pranet} (see supplementary material Table 1). 
%


%The experimental results on four different datasets (including variable-sized polyps) demonstrate that our \textit{Text-guided attention network (TGANet)} is more robust and efficient as compared to other SOTA methods. %Our proposed  TGANet can generalize well to variable-sized polyps in different datasets.


% Our network can thus understand both the size-based and the number of polyp-based feature representations that contribute to feature enhancement of any underrepresented samples (e.g., small polyp size or presence of multiple polyps) that can be present. We have also used the feature enhancement module and multi-scale feature aggregation technique to further strengthen the network. 
%  for example, in most public datasets, the presence of flat or sessile polyps are lesser than obvious and large pedunculated polyps

% Q1: What are the four encoding blocks - are they different? How they have been used?  what is the difference between each block?


Medical image segmentation plays a critical role in diagnosing and treating various diseases. Accurate and efficient segmentation of medical images can help in better decision-making. However, medical image segmentation is challenging due to the complexity and variability of medical images. We propose a prototype-based approach for medical image segmentation to address these challenges. In our proposed architecture, we first learn a small initial mask of size $64\times64$ pixels. This initial mask is then used to learn the prototype for the main object label. This prototype is subsequently used to generate the final segmentation mask of size $256\times256$ pixels. By using the prototype as a representative of the object (main segmentation class), our approach handles the variability present in the medical images and helps improve the segmentation accuracy. To further improve the accuracy and robustness of the segmentation process, we introduce a prototype bank that stores and updates a fixed number of prototypes. The stored prototypes learn different features that are complementary to the object label. These features are then used together to refine the segmentation mask further. The prototype bank allows our approach to adapt to the variability of medical images and improve the segmentation accuracy across different medical datasets. In conclusion, our proposed prototype-based approach offers a promising solution for medical image segmentation. The approach is efficient, accurate, and robust and has the potential to improve clinical decision-making and patient outcomes.


shi2022ssformer



  The main contributions of the presented work include - 1) \textit{prototype learning} to generate multiple prototypes using Prototype Generation Module (PGM), which utilizes the features learned by the Pyramid Vision Transformer (PVT) encoder and the course mask generated by the Course Mask Generation Module (CMGM), 2) \textit{Course Mask Generation Module (CMGM)} uses a Large Kernel Dilated Convolution (LKDC) block, which improves the accuracy, efficiency, and generalization capabilities of the segmentation network. 3) \textit{Encoder Feature Fusion Module (EFFM)} is used to perform multi-scale feature fusion between the different features of the PVT-encoder. It utilizes factorized convolution layers and dilated convolution layers to improve its accuracy and efficiency. 4) \textit{Prototype Mask Generation Module (PMGM)} is used to generate the final prototype mask using the prototypes generated by the PGM and the output feature map of the EFFM. 5)  We have evaluated our PrototypeLab on two publicly available polyp datasets and compared it with $16$ SOTA medical image segmentation methods.

  % The main contributions of the presented work include - 1) \textit{prototype learning} to learn different features in the context of the number of polyps presence (one or many) and size (small, medium and large), 2) \textit{course mask generation module} 3) \textit{prototype Generation Module (PGM)}, 4) \textit{\ac{OoD} generalization} to strengthen the features of the encoder and pass them to the decoder. We have evaluated our PrototypeLab  on three publicly available colon polyp datasets and compared it with 18 SOTA medical image segmentation architectures. 


  \subsection{Course mask generation module}
The Course mask generation module (CMGM) generates a course mask from the feature learned by the PVT encoder. The module begins with $X_4$, where a bilinear upsampling is applied to double its spatial dimensions. The upsampled feature map is then concatenated with $X_3$ and fed into a $3\times3$ convolution layer, followed by batch normalization and ReLU activation function. After that, the module uses a novel Large Kernel Dilated Convolution (LKDC) block, which utilizes two parallel convolution layer with large kernel sizes of $7\times7$ and $13\times13$. Next, we concatenate the output of these two layers and then followed by three parallel dilated convolution layer having a dilation rate $r = \{1, 2, 4\}$. The use of the large kernels and the dilated convolutions helps to increase the receptive field which can be beneficial for capturing more contextual information and can better handle objects of varying scales. The output of the three dilated convolution layers are concatenated and then followed by a $1\times1$ convolution layer, batch normalization and ReLU activation function. The use of our Large Kernel Dilated Convolution (LKDC) block help improve its accuracy, efficiency, and generalization capabilities of the proposed segmentation network. The output from the Large Kernel Dilated Convolution (LKDC) block is again upsampled by a factor of two and then followed by a $1\times1$ convolution layer and a sigmoid activation function to generate the course mask.

\subsection{Prototype generation module}
The prototype generation module (PGM) utilize the the features from the PVT-encoder and the course mask to generate multiple different prototypes, which are later used to generate prototype masks. The module begins with use the PVT-encoder feature $X_i$, followed by $3\times3$ convolution, batch normalization and ReLU activation. Next, an element-wise multiplication is performed between the feature map and the course mask, followed by a mask average pooling to generate a feature with dimensions $B\times256\times1\times1$, here $B$ refers to the batch size. Next, we perform a mean over the batch to generate the final prototype of size $256$. In this way, we generate four different prototype $P = \{p_1, p_2, p_3, p_4\}$ from the $X_i = \{X_1, X_2, X_3, X_4\}$

After generating four prototypes, we utilize our novel Encoder Feature Fusion Module (EFFM) to perform multi-scale feature fusion between the different features of the PVT-encoder. We begin by upsampling $X_4$ by a factor of two, concatenating it with $X_3$ and then followed by $3\times3$ Conv2D-BN-ReLU. Next, again it is upsampled by a factor of two, concatenated with $X_2$ and again followed by $3\times3$ Conv2D-BN-ReLU. Similarly, we again upsample the feature map by a factor of two, concatenated with $X_1$ and again followed by $3\times3$ Conv2D-BN-ReLU. After that, we have four parallel convolution layer, where the first layer is a $1\times1$ convolution layer. In the second layer, we have factorized the $3\times3$ convolution layer to $\{3\times1\} \{1\times3\}$ layers. Similarly for rest of the two layers, we have factorized $5\times5$ and $7\times7$. Each of the three layer is then followed by a dilated convolution layer with a dilation rate $r = \{3, 5, 7\}$. The output from the first $1\times1$ convolution layer and the three dilated convolution layers are concatenated and followed by a $1\times1$ convolution layer. Now, we utilize the output feature map of the Encoder Feature Fusion Module (EFFM) to generate the final prototype $p_5$.

\subsection{Decoder}
The decoder begin by concatenating the upsampled feature map from the Course mask generation module (CMGM) with the $X_2$ and then followed by a residual block. Next again we upsample the feature map by a factor of two and then concatenate it with the $X_1$. This is then followed by a residual block. Now, we perform upsampling operation to increase the spatial dimensions by a factor of four and then concatenate it with the original input image and then followed by residual block. The output feature map would now be used to generate the prototype masks.

\subsection{Prototype mask generation module}
The Prototype Mask Generation Module (PMGM) employs cosine similarity to generate five sets of masks by comparing the output feature map of the decoder with multiple prototypes produced in the Prototype Generation Module (PGM). 

\subsection{Final mask generation}
To generate the final segmentation mask, we concatenate the output feature map of the decoder with five set of prototype masks. The concatenated feature map is then followed by a residual block and a $1\times1$ convolution and a sigmoid activation function. 

%To further improve the accuracy and robustness of the segmentation process, we introduce a prototype bank that stores and updates a fixed number of prototypes. The stored prototypes learn different features that are complementary to the object label. These features are then used together to refine the segmentation mask further. The prototype bank allows our approach to adapt to the variability of medical images and improve the segmentation accuracy across different medical datasets.



%Medical image segmentation is critical in diagnosing and treating various diseases. Accurate and efficient segmentation of medical images can help in better decision-making. However, medical image segmentation is challenging due to the complexity and variability of medical images. We propose a prototype-based approach for medical image segmentation to address these challenges. 




\begin{figure} [!t]
    \centering
    \includegraphics[width=\textwidth]{Figures/main-architecture.jpg}
    \caption{The overall architecture of the proposed PrototypeLab. The input image is fed to the PVT-encoder to generate a coarse mask, which is combined with encoder features in the prototype generation module to generate various prototypes. Subsequently, the decoder is employed, which produces a feature map that is used to create the prototype masks. Finally, the `output mask' is generated.}
    \label{fig:prototypelab}
    % \vspace{-4mm}
\end{figure}



\begin{figure} [!h]
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/lkdc-effm.jpg}
    \caption{The diagram of the Large Kernel Dilated Convolution block and Encoder Feature Fusion Module.}
    \label{fig:lkdc_effm}
    %\vspace{-4mm}
\end{figure}

\begin{figure} [!h]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/ks-bkai.jpg}
    \caption{Qualitative results of the models trained on Kvasir-SEG and tested on BKAI-IGH.}
    \label{fig:my_label}
    %\vspace{-5mm}
\end{figure}


\begin{table}[t!]
\footnotesize
\centering
\caption{Results of models trained on Kvasir-SEG and tested on PolypGen. `Red', `Green', and `Blue' represent the best, second best and third best scores.}
 \begin{tabular} {l|c|c|c|c|c|c}
\toprule
\textbf{Method} &\textbf{mDSC}  & \textbf{mIoU}   &\textbf{Recall}& \textbf{Precision}  &\textbf{F2} &\textbf{HD}\\ 
\hline
%U-Net&0.5995 	&0.5347		&0.6829	&0.7523	&0.6105	&4.09\\
%DeepLabV3+&0.7051	&0.6389		&0.8042	&0.7659	&0.7224	&3.66\\
%PraNet&0.7258	&0.6632		&0.7999	&\textcolor{green}{0.8217}	&0.7399	&3.67\\
%MSNet&0.7112	&0.6500		&0.7570	&\textcolor{red}{\textbf{0.8641}} &0.7150	&3.72\\
TransFuse-S	&0.6956	&0.6229	&0.8079	&0.7481	&0.7180	&3.66\\
TransFuse-L&0.7273	&0.6621		&0.8060	&0.7822	&0.7404	&3.53\\
Polyp-PVT&\textcolor{blue}{0.7424}	&\textcolor{blue}{0.6763}		&0.8369	&0.7985	&0.7557	&3.44\\
UACANet&0.7185 &0.6517  &0.7972 &\textcolor{blue}{0.8007} &0.7288 &3.61\\ 
DuAT&0.7332	&0.6654	&\textcolor{green}{0.8664}	&0.7342	&0.7609	&3.48\\
CaraNet&0.6976 &0.6240	&0.8264	&0.7419	&0.7285	&3.68\\
SSFormer-S&0.7389	&0.6734	&0.8625	&0.7496	&0.7634	&\textcolor{blue}{3.43}\\
SSFormer-L&\textcolor{green}{0.7556}	&\textcolor{green}{0.6926}	&0.8530	&0.7910 &\textcolor{green}{0.7703}	&\textcolor{green}{3.37}\\
%FCBFormer~\cite{sanderson2022fcn}&0.7409 &0.6741	&\textcolor{red}{\textbf{0.8871}}	&0.7315	&0.7680	&\textcolor{red}{\textbf{3.30}}\\
UNeXt&0.4552  &0.3761  &0.6135 &0.5600 &0.4805 &4.55 \\
LDNet&0.7273	&0.6604		&0.8336	&0.7685	&0.7462	&3.53\\
TGANet&0.7030	&0.6386		&0.8030	&0.7654	&0.7177	&3.59\\
PVT-Cascade&0.7151	&0.6460		&\textcolor{blue}{0.8651} &0.7108	&0.7396	&3.48\\
\textbf{PrototypeLab}&\textcolor{red}{\textbf{0.7560}}	&\textcolor{red}{\textbf{0.6966}}	&0.8603	&0.7846 &\textcolor{red}{\textbf{0.7745}}	&\textcolor{red}{\textbf{3.35}}\\
\bottomrule
\end{tabular}
\label{tab:results}
\end{table}


 

\begin{table}[!t]
\centering
\footnotesize
\caption{The study provides model parameters, flops, and FPS for both SOTA methods and proposed PrototypeLab. `Red', `Green', and `Blue' represent the best, second best and third best scores.}
\begin{tabular}{l|c|c|c|c|c} 
\toprule
\textbf{Method} &\shortstack{\textbf{Publication}\\ \textbf{Venue}} &\textbf{Backbone} & \shortstack{\textbf{Param.}\\ (\textbf{Million)}} &\shortstack{\textbf{Flops}\\\textbf{(GMac)}} & \textbf{FPS}\\ \midrule 

%U-Net &MICCAI 2015 &-  &31.04	&54.75 &\textcolor{red}{\textbf{94.99}} \\
%DeepLabv3+ &ECCV 2018 &ResNet50 &39.76 &43.31 & \textcolor{blue}{60.47}\\
%PraNet &MICCAI 2021 &Res2Net50 &32.55 &6.93 & 29.68\\ 
%MSNet &MICCAI 2021 &Res2Net50	&29.74	&8.98 & 38.12\\
TransFuse-S & MICCAI 2021 &ResNet34 + DeiT-S &26.35 &11.5 & 34.76\\
TransFuse-L& MICCAI 2021 &ResNet50 + DeiT-B &143.74 &82.71 &37.6\\
Polyp-PVT&ArXiv 2021 &PVTv2-B2 &\textcolor{blue}{25.11} &\textcolor{green}{5.30} & 47.54 \\

UACANet &ACMMM 2021 & Res2Net50 &69.16 &31.51	&26.04 \\ 
DuAT& Arxiv 2022 &PVTv2-B2 &\textcolor{green}{24.97} &\textcolor{red}{\textbf{5.24}} & 44.56\\
CaraNet & MIIP 2022 &Res2Net101 &46.64	&11.48 &20.67 \\
SSFormer-S& MICCAI 2022 &MiT-PLD-B2 &29.57 &10.1 &49.11\\
SSFormer-L&MICCAI 2022 &MiT-PLD-B4 &66.22 &17.28 &28.21\\
%FCBFormer~\cite{sanderson2022fcn} &MIUA 2022 &PVTv2-B3 &52.96 &41.09 &18.8\\
UNeXt	&MICCAI 2022 & -	&\textcolor{red}{\textbf{1.47}} &0.5695 &\textcolor{green}{88.01} \\
LDNet& MICCAI 2022 &Res2Net50 &33.38	&33.14  &31.14\\
TGANet & MICCAI 2022 &ResNet50 &19.84	&41.88 &26.21 \\
PVT-Cascade & WACV 2023 &PVTv2-B2 &35.27	&\textcolor{blue}{8.15} &39.09\\
\textbf{PrototypeLab} & - &PVTv2-B2 &51.34 &174.87 &23.85 \\
\bottomrule
\end{tabular}
\label{algorithm_complexity}
\end{table}


\begin{table}[t!]
\footnotesize
\centering
\caption{Result of {models trained on BKAI-IGH}~\cite{lan2021neounet} and tested on PolypGen~\cite{ali2023multi}.}
 \begin{tabular} {l|c|c|c|c|c|c}
\toprule
\textbf{Method} &\textbf{mDSC}  & \textbf{mIoU}  &\textbf{Recall}& \textbf{Precision} &\textbf{F2} &\textbf{HD}\\ 
\hline
U-Net~\cite{ronneberger2015u}&0.5841	&0.5102		&0.6142	&0.7746	&0.5739	&4.36\\
DeepLabV3+~\cite{chen2018encoder}&0.6757	&0.6051		&0.7074	&0.8237	&0.6732	&4.03\\
PraNet~\cite{fan2020pranet}	&0.7330 &0.6659		&0.7825	&0.8182	&0.7391	&3.71\\
MSNet~\cite{zhao2021automatic}&0.6777	&0.6133		&0.6811	&\textcolor{red}{\textbf{0.8881}}	&0.6657	&4.06\\
TransFuse-S~\cite{zhang2021transfuse}&0.6510	&0.5720		&0.6894	&0.7952	&0.6416	&4.04\\
TransFuse-L~\cite{zhang2021transfuse}&0.6592	&0.5881		&0.6792	&0.8289	&0.6487	&4.10\\
Polyp-PVT~\cite{dong2021polyp}&\textcolor{blue}{0.7421}  &\textcolor{green}{0.6746} &0.7717	&0.8494	&\textcolor{blue}{0.7358}	&3.67\\
UACANet~\cite{kim2021uacanet}&0.7063 &0.6404  &0.7265 &\textcolor{green}{0.8519} &0.7016 &3.87 \\ 
DuAT~\cite{tang2022duat}&0.7225	&0.6553		&0.7710	&0.8081	&0.7204	&3.73\\
CaraNet~\cite{lou2022caranet}&0.6977	&0.6329		&0.7035	&\textcolor{blue}{0.8830} &0.6873	&3.99\\
SSFormer-S~\cite{wang2022stepwise}&0.7332 &0.6664		&0.7672	&0.8386	&0.7288	&3.72\\
SSFormer-L~\cite{wang2022stepwise}&\textcolor{green}{0.7426}	&\textcolor{blue}{0.6732}	&\textcolor{green}{0.7901}	&0.8209	&\textcolor{green}{0.7418}	&\textcolor{green}{3.60}\\
%FCBFormer~\cite{sanderson2022fcn}&0.7375	&0.6714		&\textcolor{green}{0.7918}	&0.8186 &0.7347	&\textcolor{red}{\textbf{3.57}}\\
UNeXt~\cite{valanarasu2022unext}&0.3484 &0.2669  &0.4519 &0.4834 &0.3492 &5.09\\
LDNet~\cite{zhang2022lesion}&0.6922 &0.6193		&0.7389	&0.8013	&0.6836	&3.83\\
TGANet~\cite{tomar2022tganet}&0.6925	&0.6206		&0.7466	&0.7833	&0.6891	&3.79\\
PVT-Cascade~\cite{rahman2023medical}&0.7271	&0.6572		&\textcolor{red}{\textbf{0.8154}} &0.7672	&\textcolor{blue}{0.7358}	&\textcolor{red}{\textbf{3.58}}\\
\textbf{PrototypeLab} &\textcolor{red}{\textbf{0.7583}} &\textcolor{red}{\textbf{0.6957}}	 &\textcolor{blue}{0.7897}	&0.8456 &\textcolor{red}{\textbf{0.7563}} &\textcolor{blue}{3.68}\\
\bottomrule
\end{tabular}
\label{tab:resultsBKAI-Polypgen}
% \vspace{-7.5mm}
\end{table}

% \begin{figure} [!t]
%     \centering
%     \includegraphics[width=0.8\textwidth]{Figures/bkai-polypgen.jpg}
%     \caption{Qualitative results of models trained BKAI-IGH and tested on PolypGen. It can be observed that PrototypeLab produces a more accurate segmentation map in all the centers from C1 to C6.}
%     \label{fig:qualitative}
%     %\vspace{-5mm}
% \end{figure}



%we introduce FANetv2, an advanced encoder decoder based network that takes a polyp image as an initial input mask, generated using Otsu thresholding and then predicts a binary segmentation mask. This predicted mask is used as the input mask for the next training epoch. FANetv2 performs two tasks: auxiliary polyp attribute classification and main polyp segmentation. The architecture takes the strength of two key mechanisms: feedback attention, using the previous epoch's predicted mask to guide the network, and a text-guided mechanism incorporating important information about polyp number and size. Together, these components enhance feature representation, improving FANetv2's overall performance. With FANetv2, we obtained a high dice coefficient of 0.9186 for BKAI-IGH and a low \ac{HD} of 2.83. Similarly, for CVC-ClinicDB, we obtained a high dice coefficient of .9481  and a low \ac{HD} of 3.19. The Source code is available at .




%\acf{CRC} is the third most common cause of cancer diagnosed in the United States and the second leading cause of cancer-related death among men and women. It is the leading cause of cancer in younger men younger than 50 years. In 2023, it was estimated that approximately 153,020 individuals were diagnosed with CRC and 52,550 died from the disease, including 19,550 cases and 3750 deaths in individuals younger than 50 years~\cite{siegel2023colorectal}. Regular screening can help detect and prevent colorectal cancer at an early stage.

% Colonoscopy is the gold standard for examining, detecting, and removing polyps. However, colonoscopy is highly operator-dependent, with high variation among the endoscopists' skills in detecting colon polyps~\cite{hetzel2010variation}. During a colonoscopy examination, the early stage of cancer is often missed. These missed polyps can develop into CRC. Fulfilling the gap between expert and non-expert endoscopists in diagnosing colon polyps has been one of the significant challenges in colonoscopy~\cite{ladabaum2013real,rees2017narrow}. The miss-rate is high due to the complex topology of organs, severe artifacts, constant organ deformation, debris and stool, etc. Even though cleansing of the bowel is done to improve detection rates of cancer and cancer precursor lesions such as polyps, the missed rate is still high, accounting for 26.8\% of polyps located on the right colon and 21.4\% of polyps on the left colon [10,12]. In addition, the missed rate for flat or sessile polyps (diminutive polyps) is grim (nearly 32.7\%). Therefore, there is a significant need to improve the screening capability of the colonoscopy procedure. 





%Block diagram of the proposed FANetv2. Here, the proposed method is fed with a polyp image and an initial input mask generated using Otsu thresholding. The network predicts a binary segmentation mask which is used as an input mask in the next training epoch. The proposed method has two tasks: \textit{an auxiliary polyp attribute classification task} and the \textit{main polyp segmentation task}. FANetv2 has two key mechanisms: a feedback attention mechanism using an input mask from the previous epoch to guide the proposed network and a text-guided mechanism incorporating crucial information regarding the number and size of polyps present within an image. These components work together to enhance the feature representation, thus improving the overall performance of the proposed FANetv2.}






































User
"Colorectal cancer (CRC) is the third most common cause of cancer diagnosed in the United States and the second leading cause of cancer-related death among men and women. Notably, it is the leading cause of cancer in younger men less  than 50 years. Colonoscopy is a gold standard for early diagnosis of colorectal cancer. However, skills among endoscopists vary significantly. Automated and accurate polyp segmentation can minimize missed rates and timely treatment of colon cancer at an early stage is possible. To address this challenge, we introduce \ac{FANetv2}, an advanced encoder-decoder network designed to automate and precisely segment polyps from colonoscopy images. Leveraging an initial input mask generated by Otsu thresholding, FANetv2 iteratively refines its binary segmentation masks through a novel feedback attention mechanism informed by the mask predictions of previous epochs. Additionally, it employs a text-guided approach that integrates critical information about the number and size of polyps to further enhance its feature representation capabilities. This dual-task strategy facilitates accurate polyp segmentation and aids in the auxiliary classification of polyp attributes, significantly boosting the model's performance. Our comprehensive evaluations on the BKAI-IGH and CVC-ClinicDB datasets demonstrate exceptional performance by achieving dice coefficients of 0.9186 and 0.9481, along with Hausdorff distances of 2.83 and 3.19, respectively. The source code for FANetv2 is available at https://github.com/xxxxx/FANetv2. 


\keywords{Polyp segmentation \and Feedback attention \and Transformer} %medical image segmentation
\end{abstract}

\section{Introduction}
\acf{CRC} is the third most common cause of cancer diagnosed in the United States and the second leading cause of cancer-related death among men and women. It is the leading cause of cancer in younger men younger than 50 years. In 2023, it was estimated that approximately 153,020 individuals were diagnosed with CRC and 52,550 died from the disease, including 19,550 cases and 3750 deaths in individuals younger than 50 years~\cite{siegel2023colorectal}. Regular screening can help detect and prevent colorectal cancer at an early stage.

Colonoscopy is the gold standard for examining, detecting, and removing polyps. However, colonoscopy is highly operator-dependent, with high variation among the endoscopists' skills in detecting colon polyps~\cite{hetzel2010variation}. During a colonoscopy examination, the early stage of cancer is often missed. These missed polyps can develop into CRC. Fulfilling the gap between expert and non-expert endoscopists in diagnosing colon polyps has been one of the significant challenges in colonoscopy~\cite{ladabaum2013real,rees2017narrow}. The miss-rate is high due to the complex topology of organs, severe artifacts, constant organ deformation, debris and stool, etc. Even though cleansing of the bowel is done to improve detection rates of cancer and cancer precursor lesions such as polyps, the missed rate is still high, accounting for 26.8\% of polyps located on the right colon and 21.4\% of polyps on the left colon [10,12]. In addition, the missed rate for flat or sessile polyps (diminutive polyps) is grim (nearly 32.7\%). Therefore, there is a significant need to improve the screening capability of the colonoscopy procedure. 




